Gosig: Scalable Byzantine Consensus on Adversarial Wide Area Network for Blockchains

Existing Byzantine fault tolerance (BFT) protocols face significant challenges in the consortium blockchain scenario. On the one hand, we can make little assumptions about the reliability and security of the underlying Internet. On the other hand, the applications on consortium blockchains demand a system as scalable as the Bit-coin but providing much higher performance, as well as provable safety. We present a new BFT protocol, Gosig, that combines crypto-based secret leader selection and multi-round voting in the protocol layer with implementation layer optimizations such as gossip-based message propagation. In particular, Gosig guarantees safety even in a network fully controlled by adversaries, while providing provable liveness with easy-to-achieve network connectivity assumption. On a wide area testbed consisting of 140 Amazon EC2 servers spanning 14 cities on five continents, we show that Gosig can achieve over 4,000 transactions per second with less than 1 minute transaction confirmation time.

==> tex_files/protocol.backup.tex <==
\section{\pname Protocol Details}
\label{protocol}

%detailedly describe the \pname protocol and explain how it achieves high security
%as well as performance.

%\subsection{Key Objectives}
%To better explain how \pname works, we firstly formally specify some important objectives that are related to
%the performance and the security of a blockchain protocol.
%For performance, we mainly optimize two metrics: the transaction throughput and the transaction latency.
%
%(1) \para{Transaction Throughput.} TPS
%
%(2) \para{Latency.} time from propagating a transaction to appearing in a published block.
%
%In order to cope with Byzantine players, the two most important security targets of \pname are:
%
%(1) \para{Consistency.} 
%The honest players in the consensus group reach agreement on the next block in each round,
%and the blockchain will not fork with overwhelming probability.
%
%(2) \para{Liveness.} 
%The protocol should continuously add non-empty blocks to the blockchain with overwhelming
%probability even if the adversary is able to \wgs{temporarily?} corrupt or disable any user 
%(by attacks such Denial of Service) at any time.

%\pname follows \cite{micali2016algorand}'s design of the cryptographic sortition to select
%a leader for each round in an unpredictable way.
%Instead of inheriting the new Byzantine agreement protocol from \cite{micali2016algorand}, which can cause
%forking on the blockchain with non-negligible probability when transient network partitioning can happen,
%\pname uses gossip-based message propagation mechanisms to achieve consensus among the honest players.

%There are two key ideas behind the design of \pname: 
%
%(1) A message with collective signatures can provide a witness proof that 
%some players have already decided to vote for a certain value, which provides more information
%useful for achieving consensus. 
%Players not only tells ``which one I agree on'' but also proves ``who also agree on it''.
%
%(2) Stochastic gossip can propagate messages efficiently as well as limit the harm of malicious
%players to the minimal.

%\wgs{I will remove 4.1, and refactor 4.2 and 4.3}

%\subsection{Protocol Outline}
%The protocol details are described in the following subsections,
%and we only give a logical outline of \pname in this part.

%\pname divides time into slots called \emph{rounds}, 
\setlength{\textfloatsep}{0pt plus 1.0pt minus 2.0pt}
\setlength{\floatsep}{0pt plus 1.0pt minus 2.0pt}
\setlength{\intextsep}{0pt plus 1.0pt minus 2.0pt}
\setlength{\abovecaptionskip}{0pt plus 3pt minus 2pt}
\setlength{\belowcaptionskip}{0pt plus 3pt minus 2pt}
\begin{figure}
\includegraphics [width=0.5\textwidth]{timeline.png}
\caption{Timeline Overview}
\label{fig:timeline}
\vspace*{0pt}
\end{figure}

We provide some details on the \pname protocol.  
\pname is a partially-synchronous protocol.
Each execution of \pname consists of a leader selection step and two subsequent \emph{stages}, as shown in Figure~\ref{fig:timeline}.  The leader selection step requires \emph{no} communication.  
Each stage takes a fixed amount of time $T_{k}$ where $k=1,2$ indicates the stage.  A typical setting of $T_{k}$s for both stages is a few seconds that is longer than the clock synchronization parameter $\Delta$.  Thus, 
all players know the current stage by referring to the global clock.  In Stage I, potential leaders disseminate their proposals to 
as many players as possible.  In Stage II, players vote for the consensus by propagating and collecting signatures and commit a block with sufficient signatures in the end.  In this section, We first describe a single round of the protocol, then introduce how we can integrate it into a blockchain. 


%\para{Round beginning: role identification.}
%At the beginning of each round $r$, some \emph{potential leaders} (may not exist) secretly know their own roles.
%One \emph{leader} (if there exist potential leaders) is determined by the protocol, but he has not been aware
%of this by then.
%
%\para{Stage I: block propogation.}
%Every potential leader constructs a block that serializes the unconfirmed transactions \he have collected so far.
%Then \he \emph{broadcasts}\wgs{Is it right to use term broadcast? use disseminate or propogate?} 
%the block with gossip described in Section~\ref{stage1}.
%On receiving the broadcast block of the round, an honest user will validate the block as well as transactions
%packed in it, and then relays the block by disseminating it
%with gossip\footnote{Optimization can be made to reduce the number of messages sent.
%We discussed this in Section~\ref{stage1}.} if the block and transactions are valid.\wgs{where to define ``valid''}
%\wgs{If I relay a block B1 proposed by p1 and then I receive a block B2 proposed by p2, 
%I find h(p2) > h(p1), i.e., p2 can't be the leader. It should be safe to neglect B2.}
%At the end of Stage I, the block proposed by the leader will be received by all honest players with high
%probability.
%
%\para{Stage II: signature aggregation.}
%Every honest user compare the owners of all the blocks \he has received in Stage I, and identify
%the one with the smallest \emph{leader score} (defined in Section~\ref{leader_election}) as the ``leader''
%(may not be the actual leader if he unluckily missed the the leader's block).
%Then he digitally signs the hash of the block proposed by the ``leader'', and disseminates the signature
%message with gossip.
%When a honest player receives an unseen signature message, if the signed block hash is the same with what
%\he has signed, then he aggregates his signature to the message, or \emph{co-signs} the message 
%(see Section~\ref{cosig}), and disseminates it with gossip.
%Otherwise, he directly disseminates it without adding his own signature.
%At the end of Stage II, with overwhelming probability every honest player will receive the message 
%containing the hash of the block proposed by the leader as well as many signatures of other honest players.
%
%\para{Round end: block publication.}
%Every honest player check the number of signatures \he has collected in Stage II for the block hash that \he
%also signed. If the number is higher than a threshold (specified in Section~\ref{block_publication}),
%the player adds the corresponding block to \his local blockchain. 
%Otherwise, he creates a special empty block to the chain.
%After the round end, with overwhelming probability, all honest users either adds the same block 
%or a special empty block to the end of the blockchain. 
%We describe how to deal with empty block in Section~\ref{block_publication}.

%\xuw{intuitions of the correctness}

\subsection{Leader Selection}
\label{leader_election}

Leader selection is the first step of \pname.
The objective of this step is to select the \emph{potential leaders} secretly.
Each player $p_i$ computes \his \emph{leader score} $L(p_i)$ using the cryptographic sortition algorithm.  Then, some players (may be zero or more than one) secretly know that they are potential leaders of the round, as 
their $L(p_i)$s are smaller than the probability parameter $q$.
Then, each potential leader $p_j$ independently proposes a value $v_{p_j} \in V$ and signs it with \his private key.
%One \emph{leader} (if there exist potential leaders) is determined by the protocol, 
%but \he doesn't need to be aware of this fact.
Note that this step requires no communication among the players.

%\para{Quick security analysis.}
Two properties of the leader selection protects the identity of the potential leaders from the adversary:
1) the signature $SIG_{p_i}$ computation involves player $p_i$'s secret key;
% which is unknown by others. 
2) Under the assumption that the hash function is a perfectly random function, the potential leader selection is uniformly random.  Also, under this completely fair process, a faulty node has no way to increase its probability of becoming a leader.  Of course, an adversary may still become a potential leader, but the following protocol ensures that the worst damage a faulty leader can cause is to make all honest players output $\bot$, affecting the liveness, but not the security guarantees.

\subsection{Two-Phase Byzantine Agreement}

After the leader selection, \pname completes the round with the following two stages. 

\subsubsection{Stage I: Proposal Broadcast}
\label{stage1}
The objective of this stage is to disseminate the value proposed by potential leaders to as many honest players as possible.
At each step, every potential leader $p_j$ sends the signature of \his proposal of $v_j$ i.e. $SIG_{p_j}(v_j)$ using gossip (details later).
On receiving a new signature message, each player verifies whether the signer of this message is indeed a potential leader. If so, \he further forwards the message using gossip protocol.

The gossip works as follows: 
We divide the stage into some fixed-length steps (typically set to a value closed to a round-trip time of the network, say, 300 ms).  At each step, a player randomly selects $m$ other players from the consensus group $G$ and sends the message along with \his signatures to them.
The parameter $m$ is a constant parameter indicating the ``gossip rate.''  Section~\ref{simulation} evaluates the trade-off between reliability and performance with different $m$, and we use $m=10$ as default.

We say the stage I achieves $\sigma$-completeness if a fraction $\sigma$ of all honest players receive 
the value proposed by every potential leader.
Our simulation shows that we can achieve $1$-completeness in stage I (every honest player receives $v_j$) with high probability. For example, in all $10,000$ simulated rounds where $N=10,000$ and $m=8$,  it only takes about 2.3 seconds for all honest players to receive a proposed block.

With leader selection, leader signature and gossip, we limit what a malicious player can achieve.  The malicious player cannot pretend to be a potential leader (everyone can verify the fact using the sortition hash), neither can it forge the signature.  In fact, the best a malicious player can do is to
cherry-pick which message to forward, but as gossip provides lots of redundancy, the faulty players cannot break \pname's security guarantees.
%neglect any messages sent by honest users(not forward them).


\subsubsection{Stage II: Signature Aggregation}
\label{stage2}

The objective of this stage for each player is to sign the value that \he receives from the potential leader
with the smallest leader score, and then disseminates \his signature to as many honest players as possible.
If a player does not receive any proposed value, \he signs a special empty value denoted by $\bot$.
Note that in this stage each honest will sign only one value.
If a player has collected more than $2f+1$ signatures of a certain proposal
during the stage II, \he can safely commit this proposal.  This is because no honest players will sign more than one value, over $2f+1$ is beyond the Byzantine fault tolerance threshold. 
%Due to limited space, we omit the optimizations we make in practice, and only logically describe the details 
%of stage II below.

%We need to gather $2f+1$ signed signatures of the same block hash in a round to ensure that this decision can be committed. Instead of sending every player's signature to others directly, which may consume a lot of network resources when the number of players is large, 

Conceptually, the stage works as the following:
Similar to stage I, each player uses gossip to propagate \his signature.
Each honest player maintains a collection $L_v = \{S_1, S_2, \cdots\}$ of all signatures it has ever seen for each proposed value $v$. 
On receiving an unseen signature $S$ for the value $v$, an honest player firstly verifies it.  If it is valid, she adds it to the collection $L_v$ with signature aggregation, 
and continues to gossip the message with aggregated signatures to $m$ randomly selected players.

%We adopt bilinear map signature~\cite{boneh2003aggregate,boneh2001short} with some
%optimization~\cite{syta2016keeping} to allow every player to aggregate all signatures signed for the same value
%privately, and the aggregated one can record who signed this block explicitly.

Similar to stage I, stage II achieves $\sigma$-completeness if each of $\sigma\in(0, 1]$ of the honest 
receives at least $2f+1$ signatures of a certain value proposed by some potential leader.
We show in Section~\ref{evaluation} that we can achieve $1$-completeness with
overwhelming probability.  This is also because the adversary is unable 
to forge signed messages or aggregated signatures.

%In our implementation, we also made optimizations such as XXX\wgs{@lpl}.
%We omit the details due to space limitations.
%
%Similar to the analysis for stage I, the adversary is unable 
%to forge signature messages or signatures. Though \he can attacks or crashes a limited number of players, \he cannot
%intercept messages sent by other users by our assumptions in Section~\ref{adversary}.


% \subsubsection{Security Analysis}
% \label{secanalysis}
% \wgs{Can omit the proof? Seems trivial.}
% \pname satisfies both $0$-agreement and consistency conditions defined in~\ref{systemmodel}.

% \par{$0$-Agreement:} Assume by contradiction that there are two honest player $p_i$ and $p_j$
% who output two different values $v_i, v_j \in V$ but $v_i \ne v_j$. By the protocol there
% are two quorums of $2f+1$ players, say $Q_1$ and $Q_2$, sign $v_i$ and $v_j$ in stage II, respectively.
% Then there is at least one honest player in $Q_1 \cap Q_2$ as $(2f + 1-f) + (2f + 1-f) = 2f + 2 > 2f+1$.
% She signs both $v_i$ and $v_j$, which is against the protocol, causing a contradiction. $\hfill \square$

% \par{Consistency:} If all honest players set their initial values the same $v\in V$, which must be proposed
% by some potential leader in stage I, then they will only sign $v$ in stage II. Any non-empty value other than $v$ can
% get at most $N-(2f + 1) = f < 2f+1$ signatures, so an honest player cannot output anything in $V$ other than $v$.
% $\hfill \square$


\subsection{Using \pname in Blockchain}
\label{toblockchain}

Gosig naturally integrates with a permissioned blockchain.

\paragraph{Transactions and Blocks. }
In applications like Bitcoin, the consensus objective for each round is a specific block containing the transactions to commit. The proposed value $v$ is a block (or the hash of the block to reduce the communication overhead). A committed block means the order and contents of all the transactions included become durable. Like all blockchains, a block also includes the hash of the previous block, meaning that the proof of the commitment of the latest block can be the proof of the entire chain.

\paragraph{Secret Leader Selection for Each Round. }
\label{leaderselectionround}
Following Algorand~\cite{micali2016algorand}, we use a number $Q^r$ to implement cryptographic sortition. 
$Q^r$ is recursively defined as
\begin{equation}
	Q^r = H(SIG_{l^r}(Q^{r-1}), r-1) \quad (r > 0)\\
\end{equation}
where $l^r$ is the $r$-round leader\footnote{
$Q^0$ is a random number. 
Please refer to \cite{micali2016algorand} for the definition of $Q^r$ when $l^r$ does not exist.}.

A player $i$'s \emph{leader score} $L^r(i)$ at round $r$ is defined as
\begin{equation}
	L^r(i) = H(SIG_i(r, Q^{r-1}))
\end{equation}
where $SIG_i(M)$ is the digital signature of message $M$ signed with $i$'s private key.
A player is a \emph{potential leader} of round $r$ if its leader score satisfies $L^r(i) < q$
where $q$ is the probability parameter with a typical value of $1/N$.

Each potential leader assembles all valid uncommitted transactions it has seen into a new block and broadcasts the block. The potential leader whose block is finally committed for this round is the actual \emph{leader} of this round.
%The $r$-round leader $l^r$ is defined as the player with the smallest $r$-round leader score.

\paragraph{Player recovery from temporary failures.  }
\label{block_inquiry}
In normal cases, blocks and signatures are broadcast to all players. If a player misses a block in round $r$ due to transient failures, it can catch up in subsequent rounds using the following procedures: 

If player $p_i$ receives a valid signature of enough signers in round $r$, but fails to receive the block itself, $i$ will check the signature and try to contact someone who signs the block to retrieve it. %It can not verify transaction validity in later rounds, thus can not generate or sign any new block, until the blocks in all previous rounds are retrieved successfully.

If player $P_i$ also fails to receive enough signatures in round $r$, it will enter the next round with round $r$ containing a temporary empty ($\bot$) block. If round $r+1$ successfully signs a block whose previous block is empty with more than $2f+1$ signers, player $i$ will commit the empty block of round $r$, or $p_i$ can retrieve the non-empty previous block and the proof from others.

%As we have analyzed, the probability that some player receives enough signature in round $r$ but round $r+1$ commits atop a temporarily empty round-$r$ block is negligible.

If player $p_i$ recovers from an extended crash period and/or data loss, it should try to retrieve all lost blocks and proofs. She can only continue participating in the protocol after she recovers all the history.  As the blocks are offline-verifiable, blocks with valid signatures from any player are sufficient for recovery.



==> tex_files/protocol_details_cryptotools.tex <==
\subsection{Cryptographic Algorithms}

In this part, we review two cryptographic algorithms we use in \pname for leader selection and reducing the space requirements for signature collection.

%\subsubsection{Leader Selection}
\subsubsection{Cryptographic sortition}
\label{leaderselection}

We inherit the \emph{cryptographic sortition} mechanism from Algorand~\cite{micali2016algorand} 
to select the leader. 
The goal of the leader selection is to randomly select a leader among a group of players who is in charge of 
proposing the new value for the group (for blockchains, the value is the next block).
The idea is to use cryptographic hash function $H(\cdot)$ as a random number generator.
The greatest challenge is to keep the election result unpredictable until the leader has disseminated
the proposed value. 
Otherwise, the adversary can launch DDoS attacks to the leader, prevent \him from broadcasting \his value,
and break the liveness of the system.

Assume there is a number $s$ shared by all players (Section~\ref{leader_election}  describes how we decide $s$ in a blockchain).  First, we compute a \emph{leader score} $L(p_i)$
%of round $r$ 
for each player $p_i$:
\begin{equation}
	L(p_i) = H(SIG_{p_i}(s))
\end{equation}
where $SIG_i(m)$ is the digital signature of message $m$ signed by $i$'s private key.
A player becomes a potential leader if \his leader score satisfies $L^s(i) < q$
where $q$ is the probability parameter. 
%The typical value of $q$ is $1/N$ ($N$ is the number of all players).
%The leader is defined as the player with the smallest leader score.

Note that without any communication, each player of the group only knows whether herself is a \emph{potential} leader,
but doesn't know if any one else in the group is a potential leader.
Only after a player broadcasts \his $SIG_{p_i}(s)$, others can verify whether \he is a potential leader.
We explain how to utilize this mechanism in Section~\ref{leaderselectionround}.

%new subsection==================================

\subsubsection{Signature Aggregation}
\label{cosig}

Our protocol requires signatures from a large portion of players.  
To reduce the storage and communication overhead of signatures,
we adopt the techniques in~\cite{boneh2001short,boneh2003aggregate} for signature aggregation.
%to reduce the size of the messages that propagate among the players
% Note that this is an optimization of performance instead of
%a necessary algorithmic building block of the consensus protocol.

The cryptographic signature of a player $p_i$ involves a hash function $H$, a generator $G$, a private key $x_i$ and a public key $V_i=G^{x_i}$. A player holding the private key $x_i$ can sign a message $M$ by computing $S_i=H(M)^{x_i}$, and others can verify the signature by checking if $e(G, S_i)$ equals $e(V_i, H(M))$ with a given bilinear map $e$. 
%To make the signature able to be aggregated, 
To know which signatures we have got,
we append an integer array $n$ of size $N$ to the signature, and by signing a message $M$, a player computes $S_i=H(M)^{x_i}$, and increments the $i$-th element of $n_{S_i}$. The combination is the signature for aggregation, and we denote this process by $sign_i(M)=(S_i,n_{S_i})$. 

An important property of the aggregated signature is that
we can accumulate it incrementally in an arbitrary order.  
Aggregating signatures is simply multiplying the BLS signature and adding the appending arrays element-wise, 
so the result is $S=H(M)^{\sum_i x_i\cdot n_S[i]}$. 
We denote the process by $aggregate(S_1, S_2,...)=(S,n_S)$. 
Suppose $(S_1, n_{S_1})$ and $(S_2, n_{S_2})$ are two aggregated signatures, 
then we can combine them by computing  $aggregated(S_1, S_2) = (S_1 * S_2, n_{S_1} + n_{S_2})$.  The integer array tells who have signed the message.  
To verify the aggregated signature, everyone can check whether $e(G, S) = e(\prod_i V_i^{n_S[i]},H(M))$. 
For safety reasons, we actually compute $H(M+V_I)$ so each player signs different messages, 
as \cite{boneh2003aggregate} points out. 
Since everyone knows others' public keys, the result is still verifiable without increasing the size of the data structure. 


